Multiscale mechanics of thermal gradient coupled graphene fracture: A molecular dynamics study

The thermo-mechanical coupling mechanism of graphene fracture under thermal gradients possesses rich applications whereas is hard to study due to its coupled non-equilibrium nature. We employ non-equilibrium molecular dynamics to study the fracture of graphene by applying a fixed strain rate under different thermal gradients by employing different potential fields. It is found that for AIREBO and AIREBO-M, the fracture stresses do not strictly follow the positive correlations with the initial crack length. Strain-hardening effects are observed for "REBO-based" potential models of small initial defects, which is interpreted as blunting effect observed for porous graphene. The temperature gradients are observed to not show clear relations with the fracture stresses and crack propagation dynamics. Quantized fracture mechanics verifies our molecular dynamics calculations. We provide a unique perspective that the transverse bond forces share the loading to account for the nonlinear increase of fracture stress with shorter crack length. Anomalous kinetic energy transportation along crack tips is observed for "REBO-based" potential models, which we attribute to the high interatomic attractions in the potential models. The fractures are honored to be more "brittle-liked" carried out using machine learning interatomic potential (MLIP), yet incapable of simulating post-fracture dynamical behaviors. The mechanical responses using MLIP are observed to be not related to temperature gradients. The temperature configuration of equilibration simulation employing the dropout uncertainty neural network potential with a dropout rate of 0.1 is reported to be the most accurate compared with the rest. This work is expected to inspire further investigation of non-equilibrium dynamics in graphene with practical applications in various engineering fields.

==> backup.tex <==
Take the green dotted line when $\Delta$T $=300$K compared with the red and blue lines for different subfigures one can deduce the effect of initial defect length on the temperature effect when a fracture occurs on graphene: when crack lengths are short, higher temperature gradients initially seem to facilitate fracture as the corresponding stresses are smaller than $\sigma_0$; as crack length increases, a high-temperature gradient seem to resist fracture as the stress difference turned to positive in subfigure {\bf E} indicating the stresses are higher with thermal gradients. Also, by observing subfigures {\bf C} and {\bf D} we observe that when defect length is around $\sim$ 3 to 4nm, it's hard to conclude the direct effect of temperature on graphene fracture, as the stress differences fluctuate. However, such a crack length regime can be identified as a fracture transiting stage: when the defect length is smaller than this value, the temperature gradients are reported to promote fracture and when the relative defect length is relatively larger the temperature gradients are observed to resist fracture. Such a phenomenon is somewhat counterintuitive as crack length may seem to "tune" the effect of thermal gradients on graphene fracture.

The initial damage pattern along the defect is also of interest. Figure \ref{damage} shows the stress $\sigma_{11}$ when the crack starts to propagate along the defect region under different temperatures with different initial lengths, where the corresponding applied strains are also marked in each subfigure. Comparing the first and last rows one observes that when the temperature gradients are at 300K, there is always some damage at the bottom of the defect regardless of initial defect length; and when there are no temperature gradients, there is always damage on the top side of the defect, regardless of defect length. Although when the temperature gradients are at 100 and 200K, the crack propagation profiles are more random, a rough trend of increasing temperature gradients leading to more damage at the bottom sides can also be deduced. We propose the following explanation for such a phenomenon: when temperatures are high, the atoms around the bottom area of the defect have higher kinetic energy, therefore having a more acute stochastic movement. The high movements induce a more sensitive response to external loading, causing the crack propagates at the bottom more compared with the same loading applied to graphene with no temperature gradients. Note that by observing the second and third columns when the initial defects are 3.1974 and 4.1812 nm such "temperature effect" becomes much more evident: when there is no thermal gradient, the crack only propagates on the top side, whereas the applied thermal gradients shift the crack propagation pattern and initiate the damage at the bottom side of the defect.

Extended from Figure \ref{stressdiffchange_to_temp}, the three-dimensional data of yield stress, initial defect size, and thermal gradient can be visualized in 2D as a contour shown in Figure \ref{contour}: the left and right subfigures stand for the yield stresses and strains, respectively. Some simple trends can be deduced from Figure \ref{stressdiffchange_to_temp}: when the initial defect length increases, the yield stresses, and strains decrease, which can also be observed in Figure \ref{stressdiffchange_to_temp}. However, an unexpected phenomenon between yield stresses and strains is detected when the initial defect length is $\sim$ 2 to 4 nm: a "zigzag-shaped" yielding stresses and strains distribution marked in the pink arrows is observed corresponding to the changing temperature gradients. Note that the phenomenon is evidently observed when the initial defect is around 2.5 nm. 

Another question arises from Figures \ref{stressdiffchange_to_temp} and \ref{contour}: Qualitatively, how does initial defect length variate the yield stresses and strains? Figure \ref{parabolic_yield} shows that both the yielding stresses and strains exhibit a concave-shaped curve with respect to the origin. As the black dashed line arrow pointed: if assume both the curves are concave, the flex points occur at yielding stress or strain corresponds to the initial defect length of around 2.5 nm, which matches the anomalous "zigzag-patterned" regime in Figure \ref{contour}
